Impact of Traffic Lights on Trajectory Forecasting of Human-driven Vehicles Near Signalized Intersections

Forecasting trajectories of human-driven vehicles is a crucial problem in autonomous driving. Trajectory forecasting in the urban area is particularly hard due to complex interactions with cars and pedestrians, and traffic lights (TLs). Unlike the former that has been widely studied, the impact of TLs on the trajectory prediction has been rarely discussed. In this work, we first identify the less studied, perhaps overlooked impact of TLs. Second, we present a novel resolution that is mindful of the impact, inspired by the fact that human drives differently depending on signal phase (green, yellow, red) and timing (elapsed time). Central to the proposed approach is Human Policy Models which model how drivers react to various states of TLs by mapping a sequence of states of vehicles and TLs to a subsequent action (acceleration) of the vehicle. We then combine the Human Policy Models with a known transition function (system dynamics) to conduct a sequential prediction; thus our approach is viewed as Behavior Cloning. One novelty of our approach is the use of vehicle-to-infrastructure communications to obtain the future states of TLs. We demonstrate the impact of TL and the proposed approach using an ablation study for longitudinal trajectory forecasting tasks on real-world driving data recorded near a signalized intersection. Finally, we propose probabilistic (generative) Human Policy Models which provide probabilistic contexts and capture competing policies, e.g., pass or stop in the yellow-light dilemma zone.

==> Literature_Review_Detail.tex <==

Models based on vehicle dynamics (Searle (1999)
Rakha et al. (2004) introduced): require traction force or engine power, and road resistance force, and not only such information is hard to observe or be estimated since they are dependent on the road conditions (which is hard to observe) on vehicle powertrain configurations and their conversion factor (thus inaccurate) which are unobservable or not accurate. Most importantly, those models have not considered traffic light state or phase, making the model not suitable for prediction of human-driven vehicles at signalized intersections real-world.

either unrealistic assumptions nor no consideration on traffic light state and phase

how human drivers react to the traffic lights.
It is quite surprising that it hasn't been thoroughly studied; we suspect that this is because (1) such model is hard to mathematically design (Searle (1999) argued that the acceleration characteristics cannot be deduced from engineering principles; and such characteristics must be acquired from field observation and measurement.) (2) lots of factors impact the human decision-making process at the signalized intersections including ~ (3) high uncertainties in human decison-making process.  Thus data-driven approach makes sense. Connected vehicles info - traffic light state and phase to bridge the gap

Akcelik and Boggs: assuming you know every in prior, not realistic, plus traffic state not considered. How do you model the aceeleration/deceleration behavior in transition? Green->yellow, yellow->red, red->green?


%%%%%%%%%%%%%%%%5
1. comparisons with existing methods (benchmark)
- benchmarking scenarios: red(how do previous algorithms solve this? cannot solve this problem), yellow->red(how do previous algorithms address the dilema zones?), red->green(with waiting time; this shows how poor previous algorithms perform without the knowledge of traffic lights) 
- Metric: how well speed profiles/distance profiles match with the actual data? how do we calculate such? R square?


The constant acceleration model has been widely used in various design processes and other study purposes due to the extreme simplicity and convenience of the practical
application of the model. [Reference obtained from Bennett and Dunn's paper]

* linear acc model:
refer to Bennett and Dunn (1995) : which talks about Samuel's algorithm, at the end of page 1

* Polynomial model by (Akcelik)

